Large Scale Substitution-based Word Sense Induction

We present a word-sense induction method based on pre-trained masked language models (MLMs), which can cheaply scale to large vocabularies and large corpora. The result is a corpus which is sense-tagged according to a corpus-derived sense inventory and where each sense is associated with indicative words. Evaluation on English Wikipedia that was sense-tagged using our method shows that both the induced senses, and the per-instance sense assignment, are of high quality even compared to WSD methods, such as Babelfy. Furthermore, by training a static word embeddings algorithm on the sense-tagged corpus, we obtain high-quality static senseful embeddings. These outperform existing senseful embeddings methods on the WiC dataset and on a new outlier detection dataset we developed. The data driven nature of the algorithm allows to induce corpora-specific senses, which may not appear in standard sense inventories, as we demonstrate using a case study on the scientific domain.

==> tables_and_figures/bass_embs.tex <==
% \begin{figure*}[t]
% \centering
%     \raisebox{-0.5\height}{\subfloat[\centering bass$_0$ closest vectors.]{{\includegraphics[width=0.9\columnwidth]{images/bass_0_black.png} }}}%
%     \qquad
%     \raisebox{-0.5\height}{\subfloat[\centering bass$_1$ closest vectors.]{{\includegraphics[width=0.9\columnwidth]{images/bass_2_black.png} }}}%
%     \caption{2D projection of our \sensewtov~- CBOW embeddings and presenting bass$_0$ and bass$_1$ closest vectors.
%     % All are musical instruments (guitars/drums/saxophone) or music related terms (rhythm/vocals). Notice \textit{keyboards} is an ambiguous terms so only keyboards$_0$ is close to bass$_0$.
%     }
%     \label{fig:bass_embs}
% \end{figure*}

==> tables_and_figures/communities_and_close_vecs/Java.tex <==
All of Java$_0$'s replacements and close embeddings relate to the Indonesia. \textit{Holland} is a possibly a replacement as Indonesia was previously known as \textit{Dutch East Indies}. Java$_1$ corresponds to the Java programming language.

\begin{table}[h]
\small
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Java$_0$} & \textbf{Java$_1$} \\
\hline
Jakarta & Eclipse \\
Indonesia & Jo \\
Bali & Apache \\
Indies & software \\
Holland & Ruby \\
\hline
\end{tabular}

\quad

\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Java$_0$} & \textbf{Java$_1$} \\
\hline
Timor$_0$ & Python$_0$ \\
Sumatra$_1$ & JavaScript \\
Sulawesi & Pascal$_2$ \\
Sumatra$_0$ & SQL \\
Kalimantan & library$_3$ \\
\hline
\end{tabular}
}
% \caption{\textit{Java}'s replacements (left) and close embeddings (right)}
\vspace{-4mm}
\end{table}


==> tables_and_figures/communities_and_close_vecs/bug.tex <==
We start with \textit{bug}'s communities as represented by their top replacements and their respective closest embeddings. Looking at both tables we can derive bug$_0$ correspond to insect. While both bug$_1$ and bug$_2$ refer to faults or defects in a computer program, a closer look reveals bug$_1$ possibly refers to a vulnerability or to being a subject to a malicious attack, while bug$_2$ is semantically closer to a software error or flaw. bug$_3$ refers to a small hidden microphone and bug$_4$ refers to the general virus term.

\begin{table}[h]
\centering
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{bug$_0$} & \textbf{bug$_1$} & \textbf{bug$_2$} & \textbf{bug$_3$} & \textbf{bug$_4$} \\
\hline
insect & problem & feature & bomb & virus \\
fly & flaws & fix & device & infection \\
beetle & hole & code & bite & crisis \\
Bugs & patch & dog & screen & disease \\
worm & mistake & software & tag & surprise \\
\hline
\end{tabular}
}

\bigskip

\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{bug$_0$} & \textbf{bug$_1$} & \textbf{bug$_2$} & \textbf{bug$_3$} & \textbf{bug$_4$} \\
\hline
bugs$_0$ & vulnerability$_2$ & bugs$_1$ & bugs$_3$ & flu$_2$ \\
beetle$_0$ & glitch & patches$_2$ & dumpster & staph \\
spider$_0$ & rootkit & bug$_1$ & laptop$_1$ & hangover \\
snake$_1$ & bugs$_1$ & updates$_1$ & footage$_1$ & nosebleed \\
worm$_0$ & virus$_2$ & patch$_2$ & cruiser$_3$ & pain$_4$ \\
\hline
\end{tabular}
}
% \caption{\textit{Bug}'s replacements (top) and close embeddings (bottom)}
\vspace{-4mm}
\end{table}

==> tables_and_figures/communities_and_close_vecs/chair.tex <==
Chair's most common senses are the executive role and a ``seat". Another, less common sense is a professor's position. This was possibly merged with chair$_1$, with ``professor" being one of its replacements.

\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{chair$_0$} & \textbf{chair$_1$} \\
\hline
head & seat \\
chairman & position \\
president & wheelchair \\
presided & professor \\
lead & table \\
\hline
\end{tabular}

\quad

\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{chair$_0$} & \textbf{chair$_1$} \\
\hline
Chair$_0$ & stool$_0$ \\
chairperson & podium$_2$ \\
chairman$_0$ & desk$_0$ \\
president$_0$ & professorship \\
Chairman$_0$ & throne$_1$ \\
\hline
\end{tabular}
}
% \caption{\textit{Chair}'s replacements (left) and close embeddings (right)}
\vspace{-4mm}
\end{table}


==> tables_and_figures/communities_and_close_vecs/mosaic-wiki.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{lllll}
\textbf{mosaic$_{w0}$} & \textbf{mosaic$_{w1}$} & \textbf{mosaic$_{w2}$} & \textbf{mosaic$_{w3}$} & \textbf{mosaic$_{w4}$} \\
marble & mixture & virus & statue & image \\
tile & landscape & var & sculpture & reproduction \\
ceramic & complex & disease & artwork & video \\
mural & mix & spread & window & scene \\
pavement & composite & yellow & plate & digital \\
\end{tabular}
}

==> tables_and_figures/communities_and_close_vecs/pound.tex <==
Reviewing \wordnet's \textit{pound} senses, there are 8 different senses that correspond to our pound$_1$ unit of money, each corresponds to a different country that uses pounds as currency. pound$_1$ is equivalent to the weight unit and pound$_2$ matches the \textit{hit/beat} verbs. Notice in ``public enclosure for dogs" sense was not found.

\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{pound$_0$} & \textbf{pound$_1$} & \textbf{pound$_2$} \\
\hline
lb & dollar & beat \\
foot & marks & punch \\
weight & coin & pump \\
ton & Mark & crush \\
kilograms & mile & attack \\
\hline
\end{tabular}

\quad

\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{pound$_0$} & \textbf{pound$_1$} & \textbf{pound$_2$} \\
\hline
lb$_0$ & rupee & smash$_2$ \\
pounds$_0$ & shilling & kick$_1$ \\
lbs$_0$ & dollar$_1$ & stomp \\
ton$_2$ & franc & slash$_0$ \\
lbs$_1$ & penny$_0$ & throw$_4$ \\
\hline
\end{tabular}
}
\vspace{-4mm}
\end{table}


==> tables_and_figures/communities_and_close_vecs/train.tex <==
Lastly we present the two senses that were found for the word \textit{train}. The first sense is analogous to the \textit{develop} or \textit{prepare} verbs and the second to the public transport.

\begin{table}[h]
\small
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{train$_0$} & \textbf{train$_1$} \\
\hline
training & railway \\
prepare & track \\
educate & rail \\
practice & line \\
qualified & railroad \\
\hline
\end{tabular}

\quad

\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{train$_0$} & \textbf{train$_1$} \\
\hline
recruit$_0$ & bus$_0$ \\
equip & tram$_1$ \\
recruit$_1$ & trains$_1$ \\
volunteer$_2$ & carriage$_0$ \\
retrain & coach$_3$ \\
\hline
\end{tabular}
}
% \caption{\textit{Train}'s replacements (left) and close embeddings (right)}
\vspace{-4mm}
\end{table}


==> tables_and_figures/community_graph.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/foundationcommunity.png}
\caption{ \textit{foundation} communities from \semeval2010.  Nodes' labels with highest degree are presented. The two largest communities are the left (blue) community, where the highest degree nodes are \textit{``organization"} and \textit{``fund"} and the rightmost (green) community, with highest degree nodes \textit{``base", ``ground", ``basis"} and \textit{``cornerstone"}.}
\label{fig:comm}
\vspace{-4mm}
\end{figure}

==> tables_and_figures/merging_senses_graph.tex <==
\begin{figure}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tikzpicture}
    \pgfplotsset{
        scale only axis,
        xmin=0, xmax=1
    }
    
    \begin{axis}[
      axis y line*=left,
      ymin=70, ymax=110,
      xlabel=Cosine similarity threshold,
      ylabel=OPP \textbackslash Accuracy,
    ]
    \addplot[smooth,mark=x,red]
      coordinates{
        (0, 91.375)
        (0.1, 92.1875)
        (0.2, 92.3125)
        (0.3, 93.5)
        (0.4, 94.25)
        (0.5, 94.75)
        (0.6, 95.94)
        (0.7, 95.5)
        (0.8, 96.3125)
        (0.9, 96.75)
        (1, 96.68)
    }; \label{OPP}
    
    \addplot[smooth,mark=o,green]
      coordinates{
        (0, 72.5)
        (0.1, 74.5)
        (0.2, 74.5)
        (0.3, 79.5)
        (0.4, 79)
        (0.5, 79.5)
        (0.6, 83)
        (0.7, 84)
        (0.8, 84.5)
        (0.9, 86)
        (1, 86)
    }; \label{accuracy}
    
    \end{axis}
    
    \begin{axis}[
      axis y line*=right,
      axis x line=none,
      ymin=0, ymax=90,
      ylabel=\% Reduction
    ]
    \addlegendimage{/pgfplots/refstyle=OPP}\addlegendentry{OPP}
    \addlegendimage{/pgfplots/refstyle=accuracy}\addlegendentry{Accuracy}
    \addplot[smooth,mark=*,blue]
      coordinates{
        (0, 80.58)
        (0.1, 79.40)
        (0.2, 76.34)
        (0.3, 70.12)
        (0.4, 60.56)
        (0.5, 48.56)
        (0.6, 35.44)
        (0.7, 21.23)
        (0.8, 8.24)
        (0.9, 1.34)
        (1, 0.00)
    }; \addlegendentry{Reduction}
    \end{axis}
    \end{tikzpicture}
    }
\caption{Performance on \ourds~dataset when close embeddings are merged. \textit{Threshold} refers the cosine similarity from which embeddings are merged. \textit{Reduction} is the percentage of the model reduction out of words with more than a single sense.}
\label{fig:merging_senses}
\vspace{-4mm}
\end{figure}

==> tables_and_figures/outlier_example.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{|c|c|}
\hline
Group Elements       & Outliers                 \\
\hline
zeus & mercury \\
hades & odysseus \\
poseidon & jesus \\
aphrodite & sparta \\
ares & delphi \\
athena & rome \\
artemis & wrath \\
\textbf{nike} & atlanta \\
\hline
\end{tabular}
\caption{Greek God example from the \textit{25-7-1-8} dataset. Nike is a distractor as it is a greek god but more likely to be used in reference to \textit{Nike, Inc.}. All elements except \textit{nike} are taken from \citet{andersen2020one}.}
\label{table:outlier_example}
\vspace{-4mm}
\end{table}
